CrisisViT: A Robust Vision Transformer for Crisis Image Classification

In times of emergency, crisis response agencies need to quickly and accurately assess the situation on the ground in order to deploy relevant services and resources. However, authorities often have to make decisions based on limited information, as data on affected regions can be scarce until local response services can provide first-hand reports. Fortunately, the widespread availability of smartphones with high-quality cameras has made citizen journalism through social media a valuable source of information for crisis responders. However, analyzing the large volume of images posted by citizens requires more time and effort than is typically available. To address this issue, this paper proposes the use of state-of-the-art deep neural models for automatic image classification/tagging, specifically by adapting transformer-based architectures for crisis image classification (CrisisViT). We leverage the new Incidents1M crisis image dataset to develop a range of new transformer-based image classification models. Through experimentation over the standard Crisis image benchmark dataset, we demonstrate that the CrisisViT models significantly outperform previous approaches in emergency type, image relevance, humanitarian category, and damage severity classification. Additionally, we show that the new Incidents1M dataset can further augment the CrisisViT models resulting in an additional 1.25% absolute accuracy gain.

==> overviewanalysis.tex <==
\section{Participant Evaluation 2019-A and 2019-B}
\ric{TREC-IS was run twice in 2019, referred to as 2019-A and 2019-B. Each of these TREC-IS editions used a different set of test events, hence we report performance on each separately. Note that performance scores are not directly comparable across editions, as the events in some editions may be easier than others, and as a general rule the later the edition the more training data will be available. 10 international research groups participated in 2019-A, contributing 35 individual runs. Similarly, 10 international research groups participated in 2019-B, providing 32 runs. However, the participating groups are different across the two editions, with 15 unique groups participating across the year.}

\ric{We report the performances of the 67 TREC Incident Streams 2019-A and 2019-B participating systems in Tables~\ref{tab:res2019A} and \ref{tab:res2019B}, respectively (evaluation notebook v2.3). Runs are grouped by research institution. The highest performing run under each metric is highlighted in bold. The Norm column indicates whether the run priority scores were subject to post-hoc max-min normalization by the organizers. Norm `-' indicates that the priority scores provided were not meaningful with or without normalization, as such we consider these runs as only tackling the information type categorization component of the task.}

\ric{Analysing Tables~\ref{tab:res2019A} and \ref{tab:res2019B}, we first note that there is no marked overlap between the best performing system under our three metric sets (Alerting, Information Feed and Prioritization). This indicates that as with 2018, participants tend to focus on either information type classification or priority estimation, but struggle to produce systems that perform well on both. For the purpose of this analysis, we will discuss each metric separately below.}

\subsection{Information Feed Performance}
\ric{Tables~\ref{tab:res2019A} and \ref{tab:res2019B} report the performance of submitted 2019-A and 2019-B systems under Accuracy All, Positive-class F1 All and Positive-class F1 Actionable metrics. In general from Tables~\ref{tab:res2019A} and \ref{tab:res2019B}, we see that information type classification performance is still on the low-end of the spectrum when considering the positive class metrics. Indeed, the highest positive-class F1 All performance observed were 25\% and 18.5\% on 2019-A and 2019-B, respectively. Meanwhile, when we only consider the actionable information types, categorization performance is lower with 18\% and 13.5\% on 2019-A and 2019-B, respectively. In general, these performance values are lower than what we would consider acceptable for deployment, and hence we can conclude that there is still substantial work needed to perform well for this task.} 

\ric{The second point of interest is that we consistently observe lower performances on 2019-B than on 2019-A. This is unexpected, as 2019-B systems had additional training examples provided to them. Hence, we might have expected performance to increase. As such, this indicates that the 2019-B events were more difficult that the 2019-A events, possibly due to the move to contemporary events (those from 2019 only).}

\ric{It is also valuable to see if there are particular patterns with regard to the systems across the events and information types. Starting with a per-event analysis, Figure~\ref{fig:categorizationPR} reports the performance of the 2019-B systems for each of the six 2019-B test events in terms of positive-class precision (a) and recall (b). Examining Figure~\ref{fig:categorizationPR} (a), we see that per event precision is strongly tied to overall system precision, i.e. precision scores tend to be roughly even across events. On the other hand, examining recall from Figure~\ref{fig:categorizationPR} (b), we observe a much greater degree of overall performance variance across systems, with the Colarado Shooting (yellow) standing out as an event where some systems had particular difficulty.} 

\ric{Next, Figure~\ref{fig:cats} provides a per-information type performance breakdown for the six actionable information types across the 2019-B systems in terms of positive-class F1. As we can see from Figure~\ref{fig:cats}, there is a high-degree of variance in terms of what actionable information types the different systems are able to identify. Although it is difficult to draw strong conclusions here, Report-EmergingThreats appears to be the category that most systems were able to at least identify some instances for, likely as it is the most common of the actionable information types (640 tweets in the test set). Meanwhile, identifying Request-SearchAndRescue requests and Report-NewSubEvent tend to be the more difficult categories, with no systems performing well. } 

\begin{figure}
    \begin{minipage}[b]{.50\linewidth}
        \centering
        \includegraphics[width=84mm]{PrecisionPerTopic}
        \subcaption{Info. Type Precision, All}\label{fig:priority_dist}
    \end{minipage}%
    \begin{minipage}[b]{.50\linewidth}
        \centering
        \includegraphics[width=80mm]{RecallPerTopic}
        \subcaption{Info. Type Recall, All}\label{fig:priority_by_type}
    \end{minipage}
    \caption{Information type categorization positive precision and recall by submitted 2019-B systems per event (all information types).}\label{fig:categorizationPR}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=160mm]{F1PerCategory.png}
  \caption{Information type categorization positive F1 performance by actionable information type per 2019-B submitted systems.}
  \label{fig:cats}
\end{figure}


\subsection{Prioritization Performance}

\ric{We next consider the performance of systems in terms of information prioritization. Tables~\ref{tab:res2019A} and \ref{tab:res2019B} report prioritization RMSE for all information types, as well as for only the actionable information types. From Tables~\ref{tab:res2019A} and \ref{tab:res2019B}, we see a promising picture, with the best systems reporting minimal RMSE scores of between 5.5\% and 7\% across both editions for all information types, with similar (but slightly higher) levels of error observed on the actionable types. This indicates that systems can be reasonably effective at estimating the priority of tweets.}

\ric{It is also worth noting that the best systems here treated prioritization as a categorization task rather than a regression task, i.e. they classified into either low, medium, high or critical priority levels before mapping to scores. In this way, their systems are more similar to the assessors. Given this, we are considering changing the track in future years to make prioritization a classification task.}




\subsection{Accumulated Alert Worth Performance}

\ric{Finally, we will comment on the Accumulated Alert Worth metrics. Although we report AAW across both years, we are hesitant to draw any conclusions from these metrics in 2019, as it is not clear that the majority of participants were aware of the impact of these metrics. In particular, it was clear when evaluating that many systems did not explicitly take into account the 0.7 score boundary (with all scores either below or above this threshold). Even with normalization, it is not clear that these scores are meaningful yet. For those few systems that did appear to make use of the full priority score range, we observed that they often returned very few alerts, which resulted in low scores. When optimising for these metrics, it is important to remember that missing important information is more costly than creating a few additional false alarms.}


\noindent A more detailed analysis of the participant runs will be provided in a separate publication. A link  will be added at \url{http://trecis.org/2019/publications.html} when that paper is published.

==> tables.tex <==
\begin{table}[t]
    \centering
    \resizebox{160mm}{!}{
    \begin{tabular}{|l|p{12cm}|p{7cm}|}
    \hline
    High-Level Information Type & Description & Example Low Level Types \\
    \hline
    Request-GoodsServices & The user is asking for a particular service or physical good. & PsychiatricNeed, Equipment, ShelterNeeded \\
Request-SearchAndRescue & The user is requesting a rescue (for themselves or others) & SelfRescue, OtherRescue\\
Request-InformationWanted & The user is requesting information & PersonsNews, MissingPersons, EventStatus\\
\hline
CallToAction-Volunteer & The user is asking people to volunteer to help the response effort & RegisterNow\\
CallToAction-Donations & The user is asking people to donate goods/money & DonateMoney, DonateGoods\\
CallToAction-MovePeople & The user is asking people to leave an area or go to another area & EvacuateNow, GatherAt\\
\hline
Report-FirstPartyObservation & The user is giving an eye-witness account & CollapsedStructure, PeopleEvacuating\\
Report-ThirdPartyObservation & The user is reporting a information from someone else & CollapsedStructure, PeopleEvacuating\\
Report-Weather & The user is providing a weather report (current or forecast) & Current, Forecast\\
Report-EmergingThreats & The user is reporting a potential problem that may cause future loss of life or damage & BuildingsAtRisk, PowerOutage, Looting\\
Report-MultimediaShare & The user is sharing images or video & Video, Images, Map\\
Report-ServiceAvailable & The user is reporting that someone is providing a service & HospitalOperating, ShelterOffered\\
Report-Factoid & The user is relating some facts, typically numerical & LandDevastated, InjuriesCount, KilledCount\\
Report-Official & An official report by a government or public safety representative & OfficialStatement, RegionalWarning, PublicAlert\\
Report-CleanUp & A report of the clean up after the event & CleanUpAction\\
Report-Hashtags & Reporting which hashtags correspond to each event & SuggestHashtags\\
\cljb{Report-News$^\star$} & The post providing/linking to continuous coverage of the event & NewsHeadline, SelfPromotion\\
\cljb{Report-NewSubEvent$^\star$} & The user is reporting a new occurrence that public safety officers need to respond to. & PeopleTrapped, UnexplodedBombFound\\
\cljb{Report-Location$^\star$} & The post contains information about the user or observation location. & Locations, GPS coordinates\\
\hline
Other-Advice & The  author is providing some advice to the public & SuggestBestPractices, CallHotline\\
Other-Sentiment & The post is expressing some sentiment about the event & Sadness, Hope, Wellwishing\\
Other-Discussion & Users are discussing the event & Causes, Blame, Rumors\\
Other-Irrelevant & The post is irrelevant, contains no information & Irrelevant\\
\cljb{Other-ContextualInformation$^\star$} & The post is generic news, e.g. reporting that the event occurred & NewsHeadline \\
\cljb{Other-OriginalEvent$^\star$} & The Responder already knows this information & KnownAlready\\
\hline

\multicolumn{3}{l}{\cljb{$^\star$ -- modified for 2019-A and 2019-B editions}} \\

    \end{tabular}}
    \caption{Ontology High-level Information Types}
    \label{tab:itypes}
\end{table}




\begin{table}[t]
    \centering
    \resizebox{160mm}{!}{
    \begin{tabular}{|l|l|l|l|c|c|}
    \hline
    Dataset & Event Name & Event Type & Source & \# Sampled & \# Assessed \\ 
    \hline
\multirow{6}{*}{Bootstrap}	&	2012	Colorado	wildfires	&	wildfire	&	CrisisLexT26~\cite{olteanu2015expect}			&	744	&	263	\\
	&	2012	Costa	Rica	Earthquake	&	earthquake	&	CrisisLexT26~\parencite{olteanu2015expect}			&	288	&	247	\\
	&	2013	Colorado	Floods	&	flood	&	CrisisLexT26~\parencite{olteanu2015expect}				&	777	&	235	\\
	&	2012	Typhoon	Pablo	&	typhoon/hurricane	&	CrisisLexT26~\parencite{olteanu2015expect}				&	649	&	244	\\
	&	2013	LA	Airport	Shooting	&	shooting	&	CrisisLexT26~\parencite{olteanu2015expect}			&	683	&	162	\\
	&	2013	West	Texas	Explosion	&	bombing	&	CrisisLexT26~\parencite{olteanu2015expect}			&	630	&	184	\\
\hline																
\multirow{15}{*}{2018}	&	2012	Guatemala	earthquake	&	earthquake	&	CrisisLexT26~\parencite{olteanu2015expect}				&	178	&	154	\\
	&	2012	Italy	earthquakes	&	earthquake	&	CrisisLexT26~\parencite{olteanu2015expect}				&	118	&	103	\\
	&	2012	Philipinnes	floods	&	flood	&	CrisisLexT26~\parencite{olteanu2015expect}				&	480	&	437	\\
	&	2013	Alberta	floods	&	flood	&	CrisisLexT26~\parencite{olteanu2015expect}				&	739	&	721	\\
	&	2013	Australia	bushfire	&	wildfire	&	CrisisLexT26~\parencite{olteanu2015expect}				&	710	&	677	\\
	&	2013	Boston	bombings	&	bombing	&	CrisisLexT26~\parencite{olteanu2015expect}				&	543	&	535	\\
	&	2013	Manila	floods	&	flood	&	CrisisLexT26~\parencite{olteanu2015expect}				&	443	&	411	\\
	&	2013	Queensland	floods	&	flood	&	CrisisLexT26~\parencite{olteanu2015expect}				&	744	&	713	\\
	&	2013	Typhoon	Yolanda	&	typhoon	&	CrisisLexT26~\parencite{olteanu2015expect}				&	629	&	564	\\
	&	2011	Joplin	tornado	&	typhoon	&	CrisisNLP	Resource	\#2~\parencite{imran2013practical}		&	152	&	96	\\
	&	2014	Chile	Earthquake	&	earthquake	&	CrisisNLP	Resource	\#1~\parencite{imran2016twitter}		&	321	&	311	\\
	&	2014	Typhoon	Hagupit	&	typhoon	&	CrisisNLP	Resource	\#1~\parencite{imran2016twitter}		&	6,696	&	4,192	\\
	&	2015	Nepal	Earthquake	&	earthquake	&	CrisisNLP	Resource	\#1~\parencite{imran2016twitter}		&	7,301	&	7,301	\\
	&	2018	FL	School	Shooting	&	shooting	&	Crawled(Twitter API)			&	1,118	&	1,118	\\
	&	2015	Paris	attacks	&	bombing	&	Crawled(GNIP)				&	2,066	&	2,066	\\
\hline																
\multirow{6}{*}{2019-A}	&	2019	Choco	Flood	&	flood	&	Crawled(Twitter API)				&	854	&	389	\\
	&	2014	California	Earthquake	&	earthquake	&	Crawled(Twitter API)				&	128	&	127	\\
	&	2013	Bohol	Earthquake	&	earthquake	&	Crawled(Twitter API)				&	646	&	582	\\
	&	2018	Florence	Hurricane	&	typhoon	&	Donated	by	participant	group	&	2,500	&	2,499	\\
	&	2017	Dallas	Shooting	&	shooting	&	Crawled(Twitter API)				&	2,500	&	2,500	\\
	&	2016	Fort	McMurray	Wildfire	&	wildfire	&	Crawled(Twitter API)			&	2,500	&	2,500	\\
\hline																
\multirow{6}{*}{2019-B}	&	2019	Alberta	Wildfires	&	wildfire	&	Crawled(Twitter API)				&	2,500	&	2,000	\\
	&	2019	Cyclone	Kenneth	&	typhoon	&	Crawled(Twitter API)				&	2,500	&	1,999	\\
	&	2019	Luzon	earthquake	&	earthquake	&	Crawled(Twitter API)				&	2,500	&	1,995	\\
	&	2019	STEM	School	Highlands	Ranch	shooting	&	shooting	&	Crawled(Twitter API)	&	2,500	&	1,238	\\
	&	2019	Durban	Easter	floods	&	flood	&	Crawled(Twitter API)			&	2,500	&	1,349	\\
	&	2019	Poway	synagogue	shooting	&	shooting	&	Crawled(Twitter API)			&	2,500	&	667	\\

    \hline
    \end{tabular}}
    \caption{TREC-IS Datasets and Labelling Statistics}
    \label{tab:events}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{r r r}
    
    \hline
    \textbf{Event Year} & \textbf{Number of TREC-IS Events} & \textbf{Number of Tweets} \\
    \hline
    
    2011 & 1 & 96 \\
    2012 & 6 & 1,448 \\
    2013 & 10 & 4,786 \\
    2014 & 3 & 4,379 \\
    2015 & 2 & 7,929 \\
    2016 & 1 & 2,000 \\
    2017 & 1 & 2,000 \\
    2018 & 2 & 3,117 \\
    2019 & 7 & 9,511 \\
    
    \hline
    \end{tabular}
    \caption{\cljb{Yearly Breakdown of Events and Tweets} }
    \label{tab:event_year}
\end{table}


\begin{table}[h]
    \centering
    \resizebox{160mm}{!}{
    \ric{
    \begin{tabular}{|l|l|p{12cm}|c|c|}
    \hline
    Source & Information & Description & \# Tweets & \% \\
    \hline
    Tweet Text & Terms/Phrases & Individual terms or phrases are information bearing, such as `trapped' or `lost power'. & 164 & 97\% \\
    & Location & The text explicitly mentions a location that is relevant to the event and the information contained is about that location & 150 & 88\% \\
    & Event Mention & The text explicitly mentions the event, making it easier to determine that this is relevant & 34 & 20\% \\
    & Time Mention & The text explicitly mentions a point in time that helped identify that the information contained was current & 10 & 6\% \\
    & Person Mention & The tweet explicitly mentions a person or twitter user account, that increases the tweet's credibility. & 10 & 6\% \\
    \hline
    Linked Content & Article/Web Page & The tweet contains a link to an external web page or news article that contains valuable information and is current. & 83 & 49\% \\
    & Tweet & The tweet links to or mentions another tweet, in this case it may the the linked tweet alone that is actionable rather than the source tweet. & 21 & 12\% \\
    & Image & The tweet contains a relevant image that is providing valuable information. & 8 & 5\% \\
    & Video & The tweet contains an embedded video that provides relevant information. & 5 & 3\% \\
    \hline
    Author & Name/Username & The tweet's username contributed to a belief that the information contained within was trustworthy, i.e. it came from an official source & 7 & 4\% \\
    \hline
    \multicolumn{5}{c}{} \\
    \hline
    \multicolumn{2}{|l|}{Regional Context Needed} & To understand the tweet some additional information (not present in the tweet) is needed, such as an understanding of geographical landmarks in the affected area & 42 & 25\% \\
    \multicolumn{2}{|l|}{Tweet is Out of Date} & The new assessor noted that based on the time-stamp of the tweet and when the information contained first became available, the information contained could be considered as out of date. & 41 & 24\% \\
    \hline
    \end{tabular}}}
    \caption{\ric{ Information contained within the Critical tweets from 2019-B. } }
    \label{tab:reswhatiscritical}
\end{table}


\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \ric{
    \begin{tabular}{|l|l|c|c|c|c|c|}
        \hline
         \multicolumn{2}{|c|}{Approach} & \multicolumn{3}{|c|}{Information Feed} & \multicolumn{2}{c|}{Prioritization} \\
        \hline
        Group & Run Name & \multicolumn{2}{|c|}{Info. Type Positive F1} & Info. Type Accuracy  & \multicolumn{2}{c|}{Priority RMSE} \\
        \hline
        & &  Actionable & All & All & Actionable & All \\
        \hline
irlabISI	&	Base		&	\textbf{0.1695}	&	\textbf{0.2825}	&	0.8521	&	0.1559	&	0.1552	\\	
irlabISI	&	Base3		&	0.1487	&	0.2642	&	0.8775	&	\textbf{0.1132}	&	0.0833	\\	
irlabISI	&	Base2		&	0.1284	&	0.2541	&	0.8812	&	0.1145	&	0.0823	\\	
CS-UCD	&	ELFB3		&	0.1180	&	0.1827	&	0.7853	&	0.1171	&	0.0603	\\	
CS-UCD	&	EL1		&	0.0970	&	0.1703	&	0.7784	&	0.1149	&	0.0617	\\	
DICE\_UPB	&	FastText		&	0.0922	&	0.1810	&	0.8501	&	0.1752	&	0.0737	\\	
CS-UCD	&	ELFB4		&	0.0918	&	0.1668	&	0.8519	&	0.1207	&	0.0623	\\	
CS-UCD	&	EL2		&	0.0884	&	0.1505	&	0.8324	&	0.1144	&	0.0633	\\	
DICE\_UPB	&	BERT		&	0.0868	&	0.2421	&	0.8809	&	0.1514	&	0.0717	\\	
NYU	&	baseline\_multi		&	0.0858	&	0.1827	&	0.8357	&	0.1223	&	0.1036	\\	
irlabISI	&	Deep		&	0.0856	&	0.1823	&	0.8765	&	\textbf{0.1132}	&	0.0833	\\	
DICE\_UPB	&	BILSTM		&	0.0814	&	0.2041	&	0.8699	&	0.1744	&	0.0757	\\	
NYU	&	baseline		&	0.0567	&	0.1287	&	0.8930	&	0.1223	&	0.1036	\\	
DICE\_UPB	&	DICE		&	0.0501	&	0.2183	&	0.8740	&	0.1532	&	0.0664	\\	
CMU	&	rf-autothre	&	0.0442	&	0.1000	&	0.8911	&	0.1890	&	0.0942	\\
NYU	&	fasttext		&	0.0440	&	0.1199	&	0.8959	&	0.1406	&	0.0722	\\	
CMU	&	rf	&0.0409	&	0.1228	&	0.8734	&	0.1571	&	0.0743	\\	
IRIT	&	rf\_gb\_threshold		&	0.0398	&	0.1886	&	0.7615	&	0.1134	&	0.0557	\\	
NYU	&	fasttext\_multi		&	0.0320	&	0.1672	&	0.8982	&	0.1306	&	0.0911	\\	
ubIS	&	-		&	0.0312	&	0.1133	&	0.3790	&	NA	&	NA	\\	
BJUTDMS	&	run2		&	0.0237	&	0.0998	&	0.5565	&	0.1150	&	\textbf{0.0563}	\\	
CMU	&	xgboost-event	&	0.0205	&	0.1516	&	0.8718	&	0.1751	&	0.0724	\\
IRIT	&	rf\_gb\_binary		&	0.0202	&	0.1513	&	0.8834	&	0.0751	&	0.0694	\\	
IRIT	&	rf\_gb\_binary\_chain		&	0.0202	&	0.1513	&	0.8834	&	0.0751	&	0.0694	\\	
IRIT	&	rf\_gb		&	0.0185	&	0.1756	&	0.8052	&	0.1134	&	0.0557	\\	
CMU	&	xgboost-extra		&	0.0106	&	0.1716	&	0.9017	&	0.1817	&	0.0732	\\
BJUTDMS	&	run1		&	0.0071	&	0.0950	&	0.6740	&	0.1343	&	0.0623	\\	
CMU	&	xgboost		&	0.0049	&	0.1638	&	0.8997	&	0.1864	&	0.0754	\\
CMU	&	rf-extra	&	0.0047	&	0.1381	&	0.8982	&	0.1886	&	0.0760	\\
ICTNET	&	-		&	0.0046	&	0.0585	&	0.6844	&	NA	&	NA	\\	
BJUTDMS	&	run3		&	0.0014	&	0.0066	&	0.6642	&	NA	&	NA	\\	
SC	&	KRun28482low		&	0	&	0.0551	&	0.8962	&	0.1723	&	0.0756	\\	
SC	&	KRun68484low		&	0	&	0.0447	&	0.9003	&	0.1756	&	0.0747	\\	
SC	&	KRun2624435		&	0	&	0.0363	&	\textbf{0.9039}	&	0.1752	&	0.0743	\\	
SC	&	KRun60002002410001		&	0	&	0.0473	&	0.8909	&	0.1731	&	0.0753	\\	
        \hline
    \end{tabular}}}
    \caption{\ric{2019-A Submitted runs under the v2.3 evaluation script. Information Feed metrics range from 0 to 1, higher is better. Prioritization metrics range from 0 to 1, lower is better. The highest performance under each metric is highlighted in bold. } }
    \label{tab:res2019A}
\end{table}

\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \ric{
    \begin{tabular}{|l|l|c|c|c|c|c|}
        \hline
         \multicolumn{2}{|c|}{Approach} & \multicolumn{3}{|c|}{Information Feed} & \multicolumn{2}{c|}{Prioritization} \\
        \hline
        Group & Run Name & \multicolumn{2}{|c|}{Info. Type Positive F1} & Info. Type Accuracy  & \multicolumn{2}{c|}{Priority RMSE} \\
        \hline
        & &  Actionable & All & All & Actionable & All \\
        \hline
CS-UCD	&	baseline	&	\textbf{0.1355}	&	0.2232	&	0.7495	&	0.0859	&	0.0668	\\
DICE\_UPB	&	BERT	&	0.1338	&	\textbf{0.2343}	&	0.8139	&	0.1558	&	0.0938	\\
CMUInformedia	&	nb	&	0.1321	&	0.2167	&	0.8605	&	\textbf{0.0788}	&	\textbf{0.0544}	\\
DICE\_UPB	&	FOCAL	&	0.1287	&	\textbf{0.2343}	&	0.8159	&	0.1416	&	0.0829	\\
CS-UCD	&	bilstmbeta	&	0.1269	&	0.1676	&	0.8378	&	0.1004	&	0.0822	\\
NYU	&	base.multi	&	0.1135	&	0.2437	&	0.7997	&	0.1836	&	0.1104	\\
DLR	&	USE\_R	&	0.1111	&	0.2232	&	0.854	&	0.1767	&	0.1019	\\
CS-UCD&		bcnelmo	&	0.1099	&	0.1721	&	0.8452	&	0.1036	&	0.0769	\\
DLR	&	BERT\_R	&	0.0998	&	0.1989	&	0.856	&	0.1834	&	0.1019	\\
NYU	&	fast.multi	&	0.0854	&	0.2256	&	\textbf{0.8808}	&	0.2153	&	0.1185	\\
CMUInformedia	&	rf2	&	0.0642	&	0.1382	&	0.8624	&	0.1025	&	0.0683	\\
CS-UCD	&	bilstmalpha	&	0.0614	&	0.171	&	0.86	&	0.1521	&	0.0893	\\
NYU	&	base.sing	&	0.0606	&	0.1373	&	0.8658	&	0.1836	&	0.1104	\\
CMUInformedia	&	rf3	&	0.0592	&	0.0813	&	0.8434	&	0.1660	&	0.2063	\\
NYU	&	fast.sing	&	0.0431	&	0.1228	&	0.8739	&	0.2085	&	0.1169	\\
UAGPLSI	&	baseline	&	0.0386	&	0.0302	&	0.8753	&	0.2067	&	0.1150	\\
UAGPLSI	&	irn	&	0.0386	&	0.0302	&	0.8753	&	0.2132	&	0.1175	\\
UAGPLSI	&	negative	&	0.0377	&	0.0278	&	0.8758	&	0.2075	&	0.1154	\\
UAGPLSI	&	all	&	0.0377	&	0.0278	&	0.8758	&	0.2138	&	0.1177	\\
ICTNET	&	dl	&	0.0347	&	0.0871	&	0.7285	&	0.1254	&	0.1451	\\
CMUInformedia	&	rf1	&	0.03	&	0.1361	&	0.8638	&	0.0815	&	0.0551	\\
IITBHU	&	run2	&	0.0275	&	0.0548	&	0.7892	&	NA	&	NA	\\
DLR	&	Fusion	&	0.0249	&	0.0939	&	0.8689	&	0.1916	&	0.1077	\\
IRIT	&	run2	&	0.0248	&	0.1725	&	0.8534	&	0.1175	&	0.0659	\\
IITBHU	&	run1	&	0.0191	&	0.0893	&	0.8139	&	0.1879	&	0.1128	\\
DLR	&	SIF\_R	&	0.016	&	0.1004	&	0.8605	&	0.2093	&	0.1129	\\
IRIT	&	run1	&	0.0151	&	0.1677	&	0.8418	&	0.1316	&	0.0911	\\
DLR	&	MeanMaxAAE\_Regression	&	0.0071	&	0.0922	&	0.8635	&	0.2111	&	0.1153	\\
IRIT	&	run4	&	0	&	0.1317	&	0.7576	&	0.1461	&	0.0775	\\
IRIT	&	run3	&	0	&	0.131	&	0.8565	&	0.1771	&	0.1028	\\
CBNU	&	C1	&	0	&	0	&	0.8788	&	NA	&	NA	\\
CBNU	&	S1	&	0	&	0	&	0.8788	&	NA	&	NA	\\
        \hline
    \end{tabular}}}
    \caption{\ric{2019-B Submitted runs under the v2.3 evaluation script. Alerting metrics range from -1 to 1, higher is better. Information Feed metrics range from 0 to 1, higher is better. Prioritization metrics range from 0 to 1, lower is better. }}
    \label{tab:res2019B}
\end{table}
